Nudging Users to Change Breached Passwords Using the Protection Motivation Theory

We draw on the Protection Motivation Theory (PMT) to design nudges that encourage users to change breached passwords. Our online experiment ($n$=$1,386$) compared the effectiveness of a threat appeal (highlighting negative consequences of breached passwords) and a coping appeal (providing instructions on how to change the breached password) in a 2x2 factorial design. Compared to the control condition, participants receiving the threat appeal were more likely to intend to change their passwords, and participants receiving both appeals were more likely to end up changing their passwords; both comparisons have a small effect size. Participants' password change behaviors are further associated with other factors such as their security attitudes (SA-6) and time passed since the breach, suggesting that PMT-based nudges are useful but insufficient to fully motivate users to change their passwords. Our study contributes to PMT's application in security research and provides concrete design implications for improving compromised credential notifications.

==> tables/pmt-action-reason.tex <==
{\footnotesize
\begin{table}[tp]
\centering
\begin{adjustbox}{width=0.8\linewidth,keepaspectratio}
\begin{tabular}{l r l r}
\textbf{Pw. Changed ($n$$=$$320$)} & \textbf{Count} & \textbf{Pw. Unchanged ($n$$=$$855$)} & \textbf{Count}\\
\cmidrule(lr){1-2} \cmidrule(lr){3-4}
to be safe  & 96 (30.0\%) &   inactive use & 282 (32.9\%)\\
bad things  & 72 (22.5\%) & no account & 169 (19.7\%) \\ 
triggered by breach & 42 (13.1\%)&  no sensitive info & 86 (10.0\%) \\
take other actions  & 41 (12.8\%) &  try and fail   & 86 (10.0\%)\\
inactive use & 20 (6.3\%) & forget to do &  78 (9.1\%) \\
to access account &  18 (5.6\%) & take other actions &  75 (8.8\%) \\
%  instructed by study  &  16 (5\%) &  unimportant account & 66 (8\%)\\
\end{tabular}
\end{adjustbox}
\caption{Top reasons for changing or not changing the breached password in the follow-up survey.}
\label{tab:pmt-action-reason}
\end{table}}

==> tables/pmt-constructs.tex <==
{\renewcommand{\arraystretch}{1.5}% for the vertical padding
\begin{table}[tp]\centering
\footnotesize
\begin{tabular}{p{0.25\linewidth}p{0.20\linewidth}p{0.10\linewidth}p{0.10\linewidth}p{0.10\linewidth}} \toprule
\textbf{Variable} &\textbf{Condition} & \textbf{Mean} & \textbf{Median} & \textbf{SD} \\ \hline
\multirow{4}{*}{Threat severity} &  Control & 4.28 & 5.00 & 0.90  \\ 
 &  Threat only & 4.37 & 5.00 & 0.79  \\ 
 &  Coping only & 4.31 & 4.50 & 0.88  \\ 
 &  Combined & 4.32 & 4.00 & 0.83  \\ 
 \hline
\multirow{4}{*}{Threat vulnerability} &  Control & 2.73 & 3.00 & 0.06  \\ 
 &  Threat only & 2.99 & 3.00 & 0.06  \\ 
 &  Coping only & 2.89 & 3.00 & 0.06  \\ 
 &  Combined & 3.01 & 3.00 & 0.06  \\ 
 \hline
 \multirow{4}{*}{Self-efficacy} &  
 Control & 3.99 & 4.00 & 1.14  \\ 
 &  Threat only & 3.96 & 4.00 & 1.15  \\ 
 &  Coping only & 4.04 & 4.00 & 1.13  \\ 
 &  Combined & 4.00 & 4.00 & 1.07  \\ 
 \hline
\multirow{4}{*}{Response efficacy} &  
 Control & 3.20 & 3.00 & 1.13  \\ 
 &  Threat only & 3.44 & 4.00 & 1.15  \\ 
 &  Coping only & 3.28 & 4.00 & 1.17  \\ 
 &  Combined & 3.55 & 4.00 & 1.13  \\ 
 \hline
\multirow{4}{*}{Response costs} &  
 Control & 1.51 & 1.00 & 0.74  \\ 
 &  Threat only & 1.52 & 1.00 & 0.79  \\ 
 &  Coping only & 1.51 & 1.00 & 0.79  \\ 
 &  Combined & 1.60 & 1.50 & 0.80  \\ 
\bottomrule
\end{tabular}
\caption{Mean, median, and standard deviation of participants' rating of the PMT constructs, divided by conditions. We adapted scales from prior work~\cite{boehmer2015determinants,story2020intent} in measuring these variables: threat severity (Q\ref{q:threat-severity-measure}), threat vulnerability (Q\ref{q:threat-vulnerability-measure}), response costs (Q\ref{q:response-cost-measure}) were measured using 5-point Likert scales, taking the median. Response efficacy (Q\ref{q:response-efficacy-measure}) and self-efficacy (Q\ref{q:self-efficacy-measure}) were measured using a single 5-point Likert-type item.}
\label{tab:pmt-construct}
\end{table}}

==> tables/pmt-intention-reason.tex <==
{\footnotesize
\begin{table}[tp]
\centering
\begin{adjustbox}{width=0.8\linewidth,keepaspectratio}
\begin{tabular}{l r l r}
\textbf{Intend to Change ($n$$=$$868$)} & \textbf{Count} & \textbf{No Intention ($n$$=$$518$)} & \textbf{Count}\\
\cmidrule(lr){1-2} \cmidrule(lr){3-4}
to be safe  & 223 (25.7\%) &   inactive use & 189 (36.5\%)\\
bad things  & 212 (24.4\%) & no account & 152 (29.3\%) \\ 
take other actions  & 181 (20.9\%) &  no sensitive info & 80 (15.4\%) \\
inactive use & 103 (11.9\%) &  forget password  & 45 (8.7\%)\\
triggered by breach  &  98 (11.3\%) & take other actions & 45 (8.7\%) \\
action good idea & 65 (7.5\%) &  unimportant password &  43 (8.3\%)\\
% reuse password &  47 (5\%) &  unimportant account & 42 (8\%)\\
\end{tabular}
\end{adjustbox}
\caption{Top reasons for intending to change or not change the breached password in the main survey.}
\label{tab:pmt-intention-reason}
\end{table}}

==> text/99_old_qual.tex <==
% \subsection{Reasoning for Changing or Not Changing Breached Passwords}
\section{Qualitative Results}
\label{subsec:qual}

We analyzed participants' open-ended responses regarding their rationales for changing or not changing breached passwords, as well as their general reactions after learning about the breach. We found that password changes occurred when participants had concerns over negative consequences or held a proactive attitude toward security. On the contrary, participants refrained from changing the password for an inactive account or resigned to inaction when they believed there was no account for which to change the password. 

% \yznote{R3: Give a little less weight to the qualitative data (and avoid quantifying it in tables such as table4), unless you’re sure that participants have given sufficient time and effort to this – its hard to tell at the moment.}

\subsection{Reasoning Behind Password Change Intention} 

To gather insights into participants' motivations and hurdles in forming password change intentions, we asked all main survey participants to explain why they intended or did not intend to change the password for the breached account (Q\ref{q:pmt-intention}). We summarize the top reasons in Table~\ref{tab:pmt-intention-reason}, differentiating between those with vs. without intention, and unpack the findings below.

\input{tables/pmt-intention-reason}

\paragraph{Reasoning for having intention.}

A common theme that exclusively applied to participants with intention to change their password was a proactive attitude toward staying safe and secure (223, 25.7\%), usually in the expression of \textit{``just to be safe,''} \textit{``to have a peace of mind,''} and \textit{``better safe than sorry.''} Such a proactive attitude could play a dominant role in participants' reasoning even when they thought the risk was limited or the account was unimportant; as one participant explained, \textit{``I'm not too concerned about my MySpace info being hacked as it was such a long time ago and any of the information I entered then would not be relevant at all now. I will however change my password if that is an option just to be on the safe side.''} 

In addition, 212 (24.4\%) participants mentioned various negative consequences that they feared could arise from being affected by the breach. The top potential consequences mentioned were personal information getting exposed, stolen, or misused (95, 10.9\%) and account compromises (86, 9.9\%). Some participants detailed how their personal information could be misused (\textit{``My LiveJournal account contains fiction I wrote that I never want to lose. The knowledge that someone could delete all that work is quite perturbing''}). Other participants highlighted possible compromises of their other accounts when credential stuffing attacks happen. This concern was particularly salient among participants who reflected that they might use the password elsewhere or had the habit of reusing passwords (47, 5.4\%); as one participant described, \textit{`` I want to change it because I use a lot of recycled passwords. Therefore, criminals could access other, more important accounts like e-mail accounts, bank accounts, my Amazon account, and other online retailer accounts.''} The finding also supports our previous quantitative results, i.e., participants who reused, or were unsure about reusing the leaked password elsewhere were much more likely to form password change intention (see Table~\ref{tab:pmt-intention-reg}).

Participants also expressed interest in taking other actions (181, 20.9\%), mostly deleting the account (119, 13.7\%). Participants might expect to change the account password in the process of deleting the account, but account deletion is usually the ultimate goal (\textit{``I don't remember making an account so I plan to do a password reset to gain access and then delete the account, if there is in fact an account as it says''}). The intention of account deletion largely depends on participants' evaluation of the account's utility and possible use; as one participant wrote, \textit{``I will probably return to the site to determine if I am still interested in maintaining an active account. If so, I will attempt to log in and change my password. If not, I will try to contact the site to get my account and associated data disabled and/or removed.''} 

% In addition, 95 (10.9\%) participants mentioned that they intended to change the password as a result of learning about the breach and being reminded that they had an account on the breached site; some explicitly highlighted that our nudges convinced them to do so even though they had received breach notifications before (\textit{``I changed my password based off of the previous screen in this survey. I had known about the breach prior to taking this survey but didn't feel prompted to change my password as I haven't used Chegg in years''}).

\paragraph{Reasoning for having no intention.}

Switching to the rationales given by participants who did not intend to change the password, the most popular reason was inactive use of the account (189, 36.5\%), i.e., the participant stopped using the account or still used it but very rarely. Comments on inactive use often came together with comments that the account did not have sensitive, important, or relevant information about themselves anymore (80, 15.4\%) or that they did not care about the account even if it was compromised (42, 8.1\%). As one participant reasoned, \textit{``This account isn't important, and I'm pretty sure I haven't logged into it in almost a decade. The information contained in it would be minimal since I never really shared personal details or provided accurate information to websites for certain questions.''} Similarly, 43 (8.3\%) participants noted that the password used for the account was an old, unimportant, or ``thrown-away'' password and had limited impact even when leaked. One participant wrote, \textit{``the password I used for it is an old and way too simple password that I don't use for my important accounts. I have used that password for some accounts like free online games but that is it.''}

Participants also commented on the practical constraints that made password change impossible or difficult. Interestingly, 152 (29.3\%) participants believed that they did not have an account with the breached site --- they did not recognize the site's name, they recognized the site but did not remember making an account, or they believed they had already deleted the account. Without an account, the advice of changing the breached password for that account becomes unrealistic, as one participant wrote, \textit{``I do not have a Quidd account so there is no password to change. Though, I do change passwords when I hear about breaches in companies I have accounts with.''}
% (\textit{``I don't have an account with MyFitnessPal -- never have, so this is kind of confusing to me''}). 
Even with an account, 45 (8.7\%) participants mentioned they forgot the password, which creates another barrier for them to change the password even when they knew password reset was an option. As one participant explained, \textit{``I don't really use this account much anymore and it's likely I don't remember my password, so I don't really want to reactivate the account just to change the password.''}

Looking at the overlapping reasons in Table~\ref{tab:pmt-intention-reason}, we found that inactive use of the account was a common theme across the board. Among participants with password change intention, 103 (11.9\%) mentioned their inactive use of the account but were still motivated to change the password due to fears of negative consequences (\textit{``I do not want hackers to have access to an account that bears my name''}) or prior negative experience (\textit{``I recently became aware of a similar hack with Chewy.com and changed my password and removed all payment data''}). Considerations of other actions were another common theme mentioned by those with (181, 20.9\%) or without (45, 8.7\%) intention, and account deletion was the top considered action for both groups. 

By contrast, whether the account has sensitive information could be a differentiating factor: 80 (15.4\%) participants without intention referred to the account's lack of sensitive information, whereas 16 (1.8\%) participants with intention were alerted by the types of information the account had about themselves. As one participant recounted, \textit{``My Pluto TV is on my Roku. Each one of those stations I have saved on my Roku can be signed in...like my National Geographic, and Discovery plus, all those channels that I pay for and have my credit card number. Now I'm worried since they got my information on my Pluto account. [I wonder] if they can get in my other account since they're all on my Roku.''}

% As one participant reasoned, \textit{``my data is very important to me. Even if it were to only be my date of birth, name, and password, I would change it. I gave my address and other important information.''}

\subsection{Reasoning Behind Password Change Action}

In the follow-up survey, we similarly asked participants to explain their reasons for changing or not changing the breached password (Q\ref{q:pmt-action}). Table~\ref{tab:pmt-action-reason} summarizes the top reasons, divided by those who changed vs. did not change the password. The themes of participants' reasoning for action mostly align with the themes of reasoning for intention but with a few notable differences, as we discuss below. 

\input{tables/pmt-action-reason}

\paragraph{Reasons for changing breached passwords.} 

Among participants who ended up changing the password, a proactive attitude toward staying safe and secure (96, 30.0\%), concerns over negative consequences (72, 22.5\%), and being alerted by the breach (42, 13.1\%) continued to be the primary motivators. Participants continued to describe other actions they took (41, 12.8\%) mostly deleting the account (23, 7.1\%) and changing the password for other accounts that were subject to password reuse or for important accounts that they cared about (15, 4.7\%). Another 18 (5.6\%) noted that they changed the password through the password reset feature to gain access to the account. However, changing the password was not their primary goal as they had other actions in mind, e.g., \textit{``I reset the password for my account, then went into settings and began the process of deleting the account.''}

\paragraph{Reasons for not changing breached passwords.} 

% Looking at the reasons given by participants who did not change their password, 
Participants continued to refer to the account's lack of use (282, 33.0\%) and lack of sensitive information (86, 10.0\%) to demonstrate the account's irrelevance or insignificance. The absence of an account continued to be a practical constraint that made password change difficult or impossible (169, 19.7\%). Consider a quote like \textit{``I haven't used the site in many years so I'm sure that my account has been deleted due to inactivity,''} it is possible that the account still exists and the participant just forgot about it. Nonetheless, 86 (10.0\%) participants confirmed that the account no longer existed as they tried to log into the account but failed. Sometimes the site did not recognize the email address they provided (\textit{``I went to Adobe site to see if I could sign in with my email address and it got [an] error message that there was no account associated with my email''}). Some participants never received the password reset email (\textit{``I requested to reset my password but they never emailed me and it wasn't in my spam or trash email folders''}). Other participants found out the site was down (\textit{``Heroes of Newerth no longer exists in any form. No website, no working game client, nothing. They basically have keys to a lock that is long gone''}). 

Failing to recover account access assured participants that they might not have an account in the first place or had deleted the account. The proliferation of data brokers might also contribute to the problem; as one participant speculated, \textit{``I don't think my Bonobos account ever existed, for example, and when I tried to reset my password, the email never came. This happened with other sites too. Maybe these sites had bought my information somehow from some other place, and therefore were able to obtain a username/email and password from me despite me never opening an account with them directly.''} Even when account recovery might be an option, some participants could not find it due to problematic interface design. As one participant recalled, \textit{``I couldn't even verify that I had a Zynga account. I think it told me to go to the specific game in question, but they have hundreds of them, and I didn't recognize them. So I have no idea what's going on.''} In line with prior work on users' struggles in account management~\cite{hammann2022account}, these friction points generate frustrations and could be detrimental even when participants had formed the intention: \textit{``I tried to log in to change the password/delete the account, but couldn't get into it. I didn't try very hard, though. When I couldn't get past the forgotten password piece, I just gave up and left it abandoned.''} 

% As much as we sought to address the costs of password change in our coping appeal (Figure~\ref{fig:coping-text}, ``It only takes a few minutes. Just follow these easy steps''), our findings show that the time and effort required in password change are highly individual-dependent, and claiming the ease of password change does not apply to everyone. 

Another notable theme among participants who did not change the password was that they had the intention but simply forgot about it or got distracted (78, 9.1\%). Participants might delay the action because they did not take password change as a priority, e.g., \textit{``I intended to change it but I procrastinated and eventually forgot all about it.''} In other cases, the forgetfulness was due to competing needs and valid challenges in their daily lives, e.g., \textit{``My best friend passed away [...] and then I flew to Arizona for her funeral. I completely forgot about this.''} Along this line, 38 (4.4\%) participants mentioned they did remember that they needed to change the password but were too busy or occupied with other duties, e.g., \textit{``I was not able to follow up, [I] have had an on-going family situation taking up my time.''} The finding about participants forgetting about or putting aside password change is not surprising --- prior work has well-documented the secondary nature of security and privacy mitigations, along with possible countermeasures such as commitment nudges~\cite{frik2019promise} and implementation planning nudges~\cite{story2020intent,story2022increasing}. However, it could be challenging to find a balance between sending useful reminders and annoying users: participants who are motivated to follow through with their intention might appreciate such reminders, but a reminder could be meaningless to those who do not see the value of password change.

\subsection{Alternative Actions Taken}
As ``take other actions'' emerged as a prominent theme among participants' responses for both intention (Table~\ref{tab:pmt-intention-reason}) and action (Table~\ref{tab:pmt-action-reason}), we unpack what these actions are by analyzing participants' responses regarding their general reactions after learning about the breach (Q\ref{q:pmt-response}). 
% In the follow-up survey, we asked participants whether they had done anything in response to learning about the breach (Q\ref{q:pmt-response}), before probing about password change specifically. 
Almost half of our participants (543, 46.2\%) said they did not do anything; the rest (632, 53.8\%) reported various actions, summarized in Table~\ref{tab:pmt-other-action}. 

\input{tables/pmt-other-action}

As participants recognized threats of password reuse, 171 (27.1\%) participants went above and beyond to change the password for other online accounts. Some participants made the change to all accounts (\textit{``I ended up changing all my passwords because I used that password for Canvas for everything else''}) while others prioritized important accounts (\textit{``I changed my Gmail password since that is the only account I'm particularly worried about''}).  In determining which accounts were at higher risk, 59 (9.3\%) participants obtained a more comprehensive list of breach records to guide their password changes (\textit{``I changed my password on Houzz, but I also checked the website, ran a few checks via Google and Firefox's password/breach checker, and found other breaches as well''}). 48 (7.6\%) participants reviewed their existing passwords to identify those that were reused and should be changed first (\textit{``I did nothing with respect to Zynga, but did spend a day updating all my passwords, including eliminating all duplicates, with my password manager''}).

In line with participants' stated intentions, deleting the breached site's account instead was another popular action (89, 14.1\%), especially for accounts that were rarely used; as one participant recounted, \textit{``After the previous survey, I did change my password. Later that day, I decided to just delete my account. I never really did use that site anyway, and it just got me thinking that I really didn't need to have any info at all on it.''} Many participants who chose to delete the account followed the logic that since the account no longer exists, they no longer need to worry about it being compromised, and the service provider now has less information about themselves. As one participant reasoned, \textit{``I was going to change my password but I decide on deleting my account instead. I don't use this account anymore and if I delete it, no one can get a hold of it.''} Nonetheless, deleting the account does not mitigate the risk of credential stuffing attacks on other accounts using the same or similar passwords. When participants mentioned deleting the account but nothing else, the key issue was whether they reused the same password for other accounts. If yes, focusing on the account with the breached site exclusively could leave out additional risks. Otherwise, deleting the account could be a reasonable and sufficient action.

Some participants expected they might still need to use the breached account in the future. In this case, they did not delete the account, instead checked or modified the content in the account to ensure there was no sensitive information (35, 5.5\%). As one participant detailed their experience, \textit{``I immediately went to my LiveJournal account, where I changed my password and the email address associated with the account.  I also confirmed that all posts which contained potentially identifying information were either deleted or set to private.''} Participants also took other actions such as searching for more information about the breached site (32, 5.1\%), reviewing and sometimes deleting other inactive accounts (27, 4.3\%), enabling two-factor authentication for important accounts (19, 3.0\%), 
% informing friends and family of the breach (10, 1.6\%), 
and researching cybersecurity topics and tools (11, 1.7\%).
% , and starting to use a password manager (9, 1.4\%). 
Even when participants did not change the password for the breached site, these alternative actions could still increase their knowledge of online self-defense and lead to better security outcomes.

Usability issues remain a major hurdle in participants' attempts to take action. Confirming our prior findings about reasons for not changing the password, 89 (14.1\%) participants documented how they tried to log into the account with the breached site but failed. Changing the password across different accounts remains a burdensome process, even with the help of tools like HIBP and password managers. In addition, participants were still apprehensive of the marginal benefits compared to the efforts required (\textit{``I only did a few of them. The whole process becomes such a pain in the ass given the various devices I have. And all of the sites in question are non-financial''}). The task became even more daunting for someone who had to do it manually (\textit{``I tried to make a list of accounts I might have out there with that email and password. I didn't change any passwords because, honestly, it was taking a long time, and I bailed on the task''}).
